Highly-confined and tunable plasmonics based on two-dimensional solid-state defect lattices

Plasmons, collective excitations of electrons in solids, are associated with strongly confined electromagnetic fields, with wavelengths far below the wavelength of photons in free space. This strong confinement promises the realization of optoelectronic devices that could bridge the size difference between photonic and electronic devices. However, despite decades of research in plasmonics, many applications remain limited by plasmonic losses, thus motivating a search for new engineered plasmonic materials with lower losses. A promising pathway for low-loss plasmonic materials is the engineering of materials with flat and energetically isolated metallic bands, which can strongly limit phonon-assisted optical losses, a major contributor to short plasmonic lifetimes. Such electronic band structures may be created by judiciously introducing an ordered lattice of defects in an insulating host material. Here, we explore this approach, presenting several low-loss, highly-confined, and tunable plasmonic materials based on arrays of carbon substitutions in hexagonal boron nitride (hBN) monolayers. From our first-principles calculations based on density functional theory (DFT), we find plasmonic structures with mid-infrared plasmons featuring very high confinements ($\lambda_{\text{vacuum}}/\lambda_{\text{plasmon}}$ exceeding 2000) and quality factors in excess of 1000. We provide a systematic explanation of how crystal structure, electronic bandwidth, and many-body effects affect the plasmonic dispersions and losses of these materials. The results are thus of relevance to low-loss plasmon engineering in other flat band systems.

==> commands.tex <==
%vectors
\newcommand{\rv}{\mathbf{r}}
\newcommand{\pv}{\mathbf{p}}
\newcommand{\kv}{\mathbf{k}}
\newcommand{\Ev}{\mathbf{E}}
\newcommand{\Dv}{\mathbf{D}}
\newcommand{\Hv}{\mathbf{H}}
\newcommand{\Bv}{\mathbf{B}}
\newcommand{\Jv}{\mathbf{J}}
\newcommand{\Rv}{\mathbf{R}}
\newcommand{\Gv}{\mathbf{G}}
\newcommand{\nablav}{\boldsymbol{\nabla}}

%symmetry vectors
\newcommand{\nv}{\mathbf{n}}

%misc
\newcommand{\tsc}[1]{\text{\textsc{#1}}}
\newcommand{\e}{\mathrm{e}}
\newcommand{\dd}{\mathrm{d}}
\newcommand{\ddb}[1]{\dd#1\,}
\newcommand{\dde}{\,\dd}
\newcommand{\iu}{\mathrm{i}}

%abbreviations
\newcommand{\ie}{i.e.,\@\xspace} %Gobble-spaces of the "small" type (small is ensured by adding \@)
\newcommand{\cf}{cf.\@\xspace}
\newcommand{\eg}{e.g.,\@\xspace}
\newcommand{\etc}{etc.\@\xspace}

%approximate \propto symbol
\newcommand{\appropto}{\mathrel{\vcenter{
			\offinterlineskip\halign{\hfil$##$\cr
				\propto\cr\noalign{\kern.2pt}\sim\cr\noalign{\kern-2.5pt}}}}}

%operators
\DeclareMathOperator{\sgn}{sgn}
\DeclareMathOperator{\interior}{int}
\DeclareMathOperator{\Tr}{Tr}
\let\Re\relax %Remove the default definition before redefining
\DeclareMathOperator{\Re}{Re}
\let\Im\relax %Remove the default definition before redefining
\DeclareMathOperator{\Im}{Im}
\newcommand{\Mod}[1]{\ (\mathrm{mod}\ #1)}

% references
\newcommand{\suppsec}{Supplemental Section\xspace}

% small solid black square, available via \smallsquare (https://tex.stackexchange.com/a/273044/113831)
\DeclareFontFamily{U}{mathb}{}
\DeclareFontShape{U}{mathb}{m}{n}{
  <-5.5> mathb5
  <5.5-6.5> mathb6
  <6.5-7.5> mathb7
  <7.5-8.5> mathb8
  <8.5-9.5> mathb9
  <9.5-11.5> mathb10
  <11.5-> mathbb12
}{}
\DeclareRobustCommand{\smallsquare}{\mathbin{\text{\usefont{U}{mathb}{m}{n}\symbol{"0D}}}}

%better alternative to \bar: \widebar (https://tex.stackexchange.com/a/336863/113831)
\DeclareFontFamily{U}{mathx}{\hyphenchar\font45}
\DeclareFontShape{U}{mathx}{m}{n}{<5> <6> <7> <8> <9> <10>
                                  <10.95> <12> <14.4> <17.28> <20.74> <24.88>
                                  mathx10}{}
\DeclareSymbolFont{mathx}{U}{mathx}{m}{n}
\DeclareFontSubstitution{U}{mathx}{m}{n}
%\DeclareMathAccent{\widebar}{0}{mathx}{"73} % commented-out due to a compilation issue
